A Difference-in-Difference Approach to Detecting AI-Generated Images

Diffusion models are able to produce AI-generated images that are almost indistinguishable from real ones. This raises concerns about their potential misuse and poses substantial challenges for detecting them. Many existing detectors rely on reconstruction error -- the difference between the input image and its reconstructed version -- as the basis for distinguishing real from fake images. However, these detectors become less effective as modern AI-generated images become increasingly similar to real ones. To address this challenge, we propose a novel difference-in-difference method. Instead of directly using the reconstruction error (a first-order difference), we compute the difference in reconstruction error -- a second-order difference -- for variance reduction and improving detection accuracy. Extensive experiments demonstrate that our method achieves strong generalization performance, enabling reliable detection of AI-generated images in the era of generative AI.

==> sec/Y_Rebuttal.tex <==
\clearpage
\onecolumn
\section{Rebuttal}
\subsection{Response to Reviewer DFYT}
\textbf{The authors compare their DID only to reconstruction-based methods in limited datasets. The fact is, there are a lot of AIGC detection methods and other more diverse dataset. The focus should not be only on reconstruction-based works. I suggest th                                 at the authors add more comparisons to other works [1,2] with more datasets [3,4].}



{\color{orange} Coming soon :)}



\textbf{There are a lot of formulas in Section 3, which are unnecessary and too redundant. I think the clear writing with necessary formulas and figures is enough.}


{\color{orange} We thank the reviewer for the suggestion regarding the presentation of Section 3. We agree that improving clarity and readability is important, especially for a broad vision audience.

We would like to clarify that the purpose of Section 3 is to provide a theoretical justification for our method, explaining why second-order reconstruction errors are effective when first-order signals become weak. We note that other reviewers explicitly found this analysis helpful and considered it a strength of the paper.

That said, we acknowledge that the exposition can be made more reader-friendly. In the revised version, we will simplify notation, reduce redundancy, and streamline the presentation, while retaining the key formulas and insights necessary to support the theoretical argument. Our goal is to make this section easier to follow without sacrificing its analytical contribution.}

\textbf{The robustness of the proposed DID is not presented, such as jpeg, blur, etc.}



{\color{orange} Thanks for the comment on robustness. We would like to gently note that JPEG robustness has already been evaluated in Section 8 of the supplementary material (due to space limitations in the main paper). During the rebuttal period we have additionally conducted blur robustness experiments, which show consistent performance trends. We will also include these results in the revised version.}

\subsection{Response to Reviewer ivYx}
Computational cost: Performing two reconstructions per image doubles the inference time compared to DIRE, which is already computationally heavy due to diffusion-based reconstruction. This limits practical deployment.

{\color{orange}
\textbf{Response:} Similar to weakness 1 in kw5y
}

Lack of real-world evaluation: The experiments are conducted on standard academic datasets. There is no validation on real-world forged images (e.g., from social media) or under adversarial attacks.


{\color{orange}
\textbf{Response:} Similar to weakness 1 in DFYT
}

\subsection{Response to Reviewer kw5y}
\textbf{My main concern is the computational cost and efficiency. The method requires performing the reconstruction process twice (getting $x^{'}$ and then $x^{''}$). As noted in the related work, methods like DIRE are already considered slow because diffusion processes are computationally heavy. By requiring a double reconstruction, the authors are essentially doubling the inference time. While the paper mentions this limitation in the discussion, there is no quantitative comparison of running time or FPS against baselines. It would be interesting to see how much slower the method is in practice, and whether the performance gain justifies the extra cost.}

{\color{orange}
\textbf{Regarding computation cost:}
We agree that DID incurs higher computational cost. In practice, this overhead is approximately 2× compared to DIRE, since the dominant cost comes from the diffusion-based reconstruction stage.

However, we would like to justify that in practical use cases, detection is typically performed on a single or a small number of images. Under this scenario, the absolute latency increase is modest. (e.g., from approximately {\color{red}XX} s to {\color{red}YY} s per image in our experiments, shown in table {\color{red}X}) and remains acceptable, especially given the gains in detection accuracy and robustness.
}

The novelty in relation to the architecture is limited. While the theoretical justification is nice, the implementation is essentially running the DIRE pipeline twice and subtracting the values. It feels like an incremental improvement over existing reconstruction-based methods. The reliance on the specific ``and'' gate fusion with a manually derived threshold (derived from the false positive rate) also feels a bit rigid. I wonder how sensitive the performance is to this thresholding strategy compared to simply concatenating the first and second-order features into a single classifier.

{\color{orange}
\textbf{Regarding novelty:}
We thank the reviewer for finding our idea “interesting and intuitive", and we appreciate the opportunity to further clarify the main source of novelty in this work.

The goal of this paper is not to introduce a new detector architecture or to improve existing network designs. Instead, the novelty of our approach is primarily theoretical and conceptual, inspired by a mathematical perspective on reconstruction-based detection. Our key insight is that higher-order reconstruction errors can capture discriminative information that first-order reconstruction errors fail to reveal, especially when first-order signals become weak.


By explicitly constructing and analyzing a second-order error term, we show that correlated perturbations can be canceled out, allowing weak but meaningful signals to re-emerge. In this sense, DID should be viewed as a principled extension of reconstruction-based detection through higher-order error analysis. As discussed in Section 5 (Discussion), our framework naturally extends to third-order and higher-order differences, revealing a broader design space for future research.


\textbf{Regarding manually derived threshold:}
Nice point, thanks for raising it. We would like to clarify that the analytically derived threshold used in the paper was not obtained through manual tuning or post-hoc adjustment. In fact, using the standard 0.5 threshold for each classifier also yields comparable performance. The choice to modify the threshold in the original submission was motivated purely by fairness in comparison, since our method requires an input to pass two classifiers simultaneously due to the AND-gate fusion, which is inherently more stringent than the single-classifier decision used by baselines.


To directly address your concern, we have added additional experiments analyzing threshold sensitivity during the rebuttal period. The results are shown in Table {\color{red} X}. As shown in the table, our method is not sensitive to the exact threshold choice and its performance remains stable across a wide range of thresholds.
}

I would also like the authors to clarify why they chose the separate classifier + "and" gate approach instead of just feeding both $\Delta(x)$ and $\Delta_2(x)$ features into a single fused classifier. Did the authors try that and did it perform worse?


{\color{orange}
Excellent point! Thank you for this insightful question. An important reason for using two separate classifiers is that the first-order and second-order reconstruction errors capture fundamentally different signals, rather than being two correlated features of the same type.


Specifically, the first-order error measures the discrepancy between the input image and its reconstruction. Therefore, it reflects how far the image lies from the learned generative manifold. In contrast, the second-order error characterizes the stability of reconstruction errors across successive reconstructions. It reflects the robustness of the reconstruction process itself rather than the absolute reconstruction discrepancy. Therefore, using separate classifiers allows us to explicitly model these two qualitatively different signals and maintain interpretability. 

That said, feeding both $\Delta(x)$ and $\Delta_2(x)$ features into a single fused classifier is also a reasonable design. We have conducted additional experiment (shown in Table {\color{red}X}) {\color{red}[JZ] If possible, shall we can put this paragraph first? As the reviewer asks for this experiment, the previous two paragraph looks like we are not delighted to provide this experiment.}

{\color{cyan}If experiment result is comparable, we keep the `and' gate design for intepretability.}
}


%Existing reconstruction-based methods almost exclusively focus on first-order reconstruction error, implicitly assuming that this quantity remains informative across regimes. Our analysis shows that this assumption breaks down when the generator becomes strong, as the first-order error is dominated by stochastic perturbations introduced during reconstruction.

% By explicitly constructing and analyzing a second-order error term, we demonstrate that correlated perturbations can be canceled out, allowing weak but meaningful signals—related to the distance between real images and the learned generative manifold—to re-emerge. In this sense, DID should be viewed not as an architectural modification of existing detectors, but as a reframing of reconstruction-based detection through the lens of higher-order error analysis.

%We further emphasize that this insight is general and not limited to the second-order case. As discussed in the paper, the same reasoning naturally extends to third-order and higher-order errors, suggesting a broader design principle rather than a one-off incremental improvement. We will revise the manuscript to make this conceptual contribution more explicit.


% requires: \usepackage{booktabs,multirow}
% (optional) \usepackage{caption}  % if you want \captionof in minipage; here we use sub-captions via plain text.

% numbers now formatted to TWO decimals for both ACC and AP (ACC/AP)

\begin{table*}[!t]
\caption{Accuracy / AP (shown as \textbf{ACC/AP}) of different detectors under two training settings: \textbf{GenImage (train)} (left block) and \textbf{ImageNet (ckpt)} (right block). Best (by \textbf{ACC}) in \textbf{bold}, second best \underline{underlined}. All averages are computed from raw values and then rounded to two decimals.}
\label{tab:genimage_vs_imagenet_accap}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{ll| c c c c | c c c c}
\toprule
\multicolumn{2}{c|}{\textbf{Train set \& Gen. model}} &
\multicolumn{4}{c|}{\textbf{GenImage (train)}} &
\multicolumn{4}{c}{\textbf{ImageNet (ckpt)}} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}
\textbf{Eval set} &
\textbf{Gen. model} &
\textbf{Ours$_{0.29}$} &
\textbf{Ours$_{0.5}$} &
\textbf{Effort} &
\textbf{DDA} &
\textbf{Ours$_{0.29}$} &
\textbf{Ours$_{0.5}$} &
\textbf{Effort} &
\textbf{DDA} \\
\midrule
\multirow{9}{*}{GenImage}
 & ADM        & \underline{99.90/1.00} & \textbf{100.00/1.00} & 98.55/1.00 & 99.30/1.00 & \underline{99.20/1.00} & \textbf{99.50/1.00} & 86.30/0.99 & 98.30/1.00 \\
 & BigGAN     & \underline{99.90/1.00} & \textbf{99.95/1.00}  & 95.45/0.99 & 98.70/1.00 & \underline{99.10/1.00} & \textbf{99.40/1.00} & 80.15/0.85 & 98.50/1.00 \\
 & GLIDE      & \underline{99.90/1.00} & \textbf{100.00/1.00} & 98.35/1.00 & 99.20/1.00 & \underline{99.20/1.00} & \textbf{99.50/1.00} & 85.85/0.97 & 97.50/1.00 \\
 & Midjourney & \textbf{99.70/1.00}    & \textbf{99.70/1.00}  & 57.25/0.75 & \underline{54.95/0.83} & \underline{99.20/1.00} & \textbf{99.50/1.00} & 57.00/0.62 & 56.15/0.79 \\
 & SD-v1.4    & \underline{99.45/1.00} & \textbf{99.50/1.00}  & 86.70/0.98 & 72.81/0.96 & \underline{99.20/1.00} & \textbf{99.50/1.00} & 85.30/0.96 & 82.91/0.97 \\
 & SD-v1.5    & \textbf{99.50/1.00}    & \underline{99.40/1.00} & 83.95/0.97 & 72.65/0.96 & \underline{99.20/1.00} & \textbf{99.50/1.00} & 84.75/0.95 & 83.60/0.97 \\
 & VQDM       & \textbf{99.90/1.00}    & \textbf{99.90/1.00}  & 97.00/1.00 & \underline{99.50/1.00} & \underline{99.20/1.00} & \textbf{99.50/1.00} & 86.45/0.99 & 98.55/1.00 \\
 & Wukong     & \textbf{99.20/1.00}    & \underline{99.15/1.00} & 83.05/0.97 & 74.50/0.96 & \underline{99.20/1.00} & \textbf{99.45/1.00} & 84.40/0.95 & 84.10/0.97 \\
\cmidrule(lr){2-10}
 & Avg.       & \underline{99.68/1.00} & \textbf{99.70/1.00}  & 87.54/0.96 & 83.95/0.96 & \underline{99.19/1.00} & \textbf{99.48/1.00} & 81.27/0.91 & 87.45/0.96 \\
\midrule
\multirow{7}{*}{GenDen+Img}
 & BigGAN     & \textbf{99.95/1.00} & \textbf{99.95/1.00} & 98.55/1.00 & \underline{99.20/1.00} & \underline{99.85/1.00} & \textbf{99.90/1.00} & 99.70/1.00 & 99.45/1.00 \\
 & CRN        & \textbf{99.95/1.00} & \textbf{99.95/1.00} & 98.15/1.00 & \underline{98.45/1.00} & \underline{99.85/1.00} & \textbf{99.90/1.00} & 98.80/1.00 & 99.35/1.00 \\
 & DeepFake   & \textbf{99.65/1.00} & \underline{99.45/1.00} & 96.35/1.00 & 99.20/1.00 & \textbf{99.50/1.00} & \underline{99.30/1.00} & 96.75/1.00 & 99.30/1.00 \\
 & GauGAN     & \textbf{99.95/1.00} & \textbf{99.95/1.00} & 97.45/1.00 & \underline{99.35/1.00} & \underline{99.85/1.00} & \textbf{99.90/1.00} & 99.65/1.00 & 99.60/1.00 \\
 & IMLE       & \textbf{99.95/1.00} & \textbf{99.95/1.00} & 98.70/1.00 & \underline{97.70/1.00} & \underline{99.85/1.00} & \textbf{99.90/1.00} & 99.75/1.00 & 99.40/1.00 \\
 & StarGAN    & \textbf{99.95/1.00} & \textbf{99.95/1.00} & 98.50/1.00 & \underline{99.35/1.00} & \underline{99.85/1.00} & \textbf{99.90/1.00} & 99.65/1.00 & 99.60/1.00 \\
\cmidrule(lr){2-10}
 & Avg.       & \textbf{99.90/1.00} & \underline{99.87/1.00} & 97.95/1.00 & 98.88/1.00 & \textbf{99.79/1.00} & \underline{99.78/1.00} & 99.05/1.00 & 99.45/1.00 \\
\midrule
\multirow{6}{*}{New-JPG}
 & KAN32      & \textbf{99.60/1.00} & \textbf{99.60/1.00} & 63.85/0.85 & \underline{57.10/0.80} & \underline{99.30/1.00} & \textbf{99.55/1.00} & 80.75/0.93 & 59.05/0.78 \\
 & Play2      & \textbf{99.60/1.00} & \underline{99.55/1.00} & 67.05/0.88 & 81.55/0.96 & \underline{99.30/1.00} & \textbf{99.60/1.00} & 83.95/0.94 & 87.00/0.96 \\
 & SDXL2      & \textbf{99.60/1.00} & \underline{99.50/1.00} & 66.85/0.88 & 67.70/0.90 & \underline{99.25/1.00} & \textbf{99.55/1.00} & 85.00/0.95 & 76.30/0.91 \\
 & Stable2    & \textbf{99.65/1.00} & \underline{99.55/1.00} & 81.20/0.96 & 69.20/0.91 & \underline{99.35/1.00} & \textbf{99.65/1.00} & 90.60/0.98 & 75.50/0.92 \\
 & Vega2      & \textbf{98.90/1.00} & \underline{98.75/1.00} & 57.50/0.76 & 76.90/0.94 & \underline{99.25/1.00} & \textbf{99.55/1.00} & 79.85/0.92 & 80.80/0.94 \\
\cmidrule(lr){2-10}
 & Avg.       & \textbf{99.47/1.00} & \underline{99.39/1.00} & 67.29/0.87 & 70.49/0.90 & \underline{99.29/1.00} & \textbf{99.58/1.00} & 84.03/0.95 & 75.73/0.90 \\
\midrule
\multirow{3}{*}{ImageNet}
 & ADM        & \textbf{99.65/1.00} & \textbf{99.65/1.00} & 97.20/1.00 & \underline{99.05/1.00} & \underline{99.85/1.00} & \textbf{99.90/1.00} & 99.40/1.00 & 99.55/1.00 \\
 & SD-v1      & \textbf{99.35/1.00} & \underline{98.70/1.00} & 84.70/0.96 & 71.05/0.96 & \underline{99.85/1.00} & \textbf{99.90/1.00} & 98.10/1.00 & 83.45/0.99 \\
\cmidrule(lr){2-10}
 & Avg.       & \textbf{99.50/1.00} & \underline{99.17/1.00} & 90.95/0.98 & 85.05/0.98 & \underline{99.85/1.00} & \textbf{99.90/1.00} & 98.75/1.00 & 91.50/0.99 \\
\midrule
\multicolumn{2}{l|}{Total average} &
\textbf{99.68/1.00} & \underline{99.62/1.00} & 86.02/0.95 & 85.11/0.96 &
\underline{99.45/1.00} & \textbf{99.63/1.00} & 88.67/0.95 & 88.47/0.96 \\
\bottomrule
\end{tabular}
\end{table*}

